COCO-LM: Correcting and Contrasting Text Sequences for Language Model Pretraining

We present a self-supervised learning framework, COCO-LM, that pretrains Language Models by COrrecting and COntrasting corrupted text sequences. Following ELECTRA-style pretraining, COCO-LM employs an auxiliary language model to corrupt text sequences, upon which it constructs two new tasks for pretraining the main model. The first token-level task, Corrective Language Modeling, is to detect and correct tokens replaced by the auxiliary model, in order to better capture token-level semantics. The second sequence-level task, Sequence Contrastive Learning, is to align text sequences originated from the same source input while ensuring uniformity in the representation space. Experiments on GLUE and SQuAD demonstrate that COCO-LM not only outperforms recent state-of-the-art pretrained models in accuracy, but also improves pretraining efficiency. It achieves the MNLI accuracy of ELECTRA with 50% of its pretraining GPU hours. With the same pretraining steps of standard base/large-sized models, COCO-LM outperforms the previous best models by 1+ GLUE average points.

==> Figures/attn_study.tex <==

\begin{figure}[t]
\vspace{-0.5cm}
\centering
\includegraphics[width=0.3\textwidth]{Figures/attn_plot.pdf}
\caption{The entropy of learned attention weights (after softmax) in different Transformer layers. The x-axis marks the layer index (smaller means closer to input tokens). The entropy is averaged on all tokens in the MNLI corpus without fine-tuning.
}
\label{fig:attn_study}
\vspace{-0.3cm}
\end{figure}

==> Figures/clm.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{Figures/replace_correct.pdf}
\caption{Overview of Replaced Token Correction (RTC). A sequence is partially masked out and fed into a shallow masked language model (MLM) that predicts the masked tokens. The MLM predicted sequence is then fed into \model that recovers the original sequence by correcting the replaced tokens.\cx{single column? merge with Fig 2 to one two-col figure?}} 
\label{fig:replace_correct}
\end{figure*}


==> Figures/cls_study.tex <==

\begin{figure}[t]
\begin{subfigure}[t]{0.235\textwidth}
\centering
	\includegraphics[width=\textwidth]{Figures/few_shot_plot_m.pdf}
	\caption{MNLI-m\label{fig:few_shot_m}}
\end{subfigure}%
~
\begin{subfigure}[t]{0.235\textwidth}
\centering
	\includegraphics[width=\textwidth]{Figures/few_shot_plot_mm.pdf}
	\caption{MNLI-mm\label{fig:few_shot_mm}}
\end{subfigure}
\caption{Few-shot accuracy on MNLI with a fraction of MNLI training set used (x-axes). The error bars mark the max/min and the solid lines are the average of five fine-tuning runs. 
% \cx{This one needs redraw and add some points}
}
\label{fig:few_shot_study}
\vspace{-0.3cm}
\end{figure}

==> Figures/cls_training.tex <==


\begin{figure}[t]
% \subfigcapmargin=10pt
\centering
\begin{subfigure}[t]{0.235\textwidth}
\centering
% 	\includegraphics[width=\textwidth]{Figures/few_shot_plot_mm.pdf}
	\includegraphics[width=\textwidth]{Figures/no_contrast_cosine.pdf}
	\caption{Without SCL}
\end{subfigure}%
~
\begin{subfigure}[t]{0.235\textwidth}
\centering
% 	\includegraphics[width=\textwidth]{Figures/few_shot_plot_m.pdf}
	\includegraphics[width=\textwidth]{Figures/contrast_cosine.pdf}
	\caption{With SCL}
\end{subfigure}

\caption{The cosine similarity between the \texttt{[CLS]} embeddings of positive and negative sequence pairs during pretraining. 
% The x-axes mark the training steps.
}\label{fig:scl_curve}
\end{figure}


==> Figures/cls_tsne.tex <==


\begin{figure}[t]
\begin{subfigure}[t]{0.4\textwidth}
\centering
	\includegraphics[width=\textwidth]{Figures/cls_no_contrast.pdf}
	\caption{Without SCL\label{fig:no_scl}}
\end{subfigure}%
~
\begin{subfigure}[t]{0.4\textwidth}
\centering
	\includegraphics[width=\textwidth]{Figures/cls_contrast.pdf}
	\caption{With SCL\label{fig:scl}}
\end{subfigure}

\caption{The t-SNE plots of learned sequence representations with or without SCL. The points are sampled from the most semantically similar sentences pairs from STS-B (with $5$-score labels). The \texttt{[CLS]} embeddings are obtained without fine-tuning. Some similar pairs are random selected and marked by the same shapes.
} 
\label{fig:scl_tsne}
\end{figure}

==> Figures/efficiency.tex <==

\begin{figure}[t]
% \subfigcapmargin=10pt
\centering
\begin{subfigure}[t]{0.235\textwidth}
\centering
% 	\label{fig:efficency_m}
	\includegraphics[width=\textwidth]{Figures/efficiency_m.pdf}
	\caption{MNLI-m}
\end{subfigure}%
~
\begin{subfigure}[t]{0.235\textwidth}
\centering
% 	\label{fig:efficency_mm}
	\includegraphics[width=\textwidth]{Figures/efficiency_mm.pdf}
	\caption{MNLI-mm}
\end{subfigure}
\caption{\model Base accuracy on MNLI Dev. sets (y-axes) at different pretraining hours on four DGX-2 nodes ($64$ V100 GPUs). 
The final training hours and accuracy of RoBERTa (ours) and ELECTRA (Ours) are measured in the exact same settings and computing environments.
}
% \vspace{-0.3cm}
	\label{fig:efficency}
\end{figure}


==> Figures/few_shot.tex <==

% \begin{figure}[t]
% % \subfigcapmargin=10pt
% \centering
% \includegraphics[width=0.5\textwidth]{Figures/few_shot_plot.pdf}
% \caption{
% }
% \label{fig:few_shot_study}
% \end{figure}

\begin{figure}[t]
% \subfigcapmargin=10pt
\centering
\begin{subfigure}[t]{0.25\textwidth}
\centering
	\label{fig:few_shot_m}
	\includegraphics[width=\textwidth]{Figures/few_shot_plot_m.pdf}
	\caption{MNLI-m}
\end{subfigure}%
~
\begin{subfigure}[t]{0.25\textwidth}
\centering
	\label{fig:few_shot_mm}
	\includegraphics[width=\textwidth]{Figures/few_shot_plot_mm.pdf}
	\caption{MNLI-mm}
\end{subfigure}
\caption{.}
\end{figure}

==> Figures/scl.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{Figures/contrast.pdf}
\caption{Overview of Sequence Contrastive Learning (SCL). Two different transformations (\eg, MLM Replacement and Random Subsequence Extraction) are applied to the original sequences. A contrastive loss is used to encourage the model to correctly identify sequence pairs that are transformed from the same sequences.} 
\label{fig:contrast}
\end{figure*}


==> Figures/self_learn_tsb.tex <==

\begin{figure}[t]
% \subfigcapmargin=10pt
\centering
\centering
% 	\label{fig:efficency_m}
	\includegraphics[width=\textwidth]{Figures/efficiency_m.pdf}
\caption{\model Replacement detection accuracy of \model when pretrained using: \textit{Random}ly replaced tokens, sampled from a pretrained and Fixed auxiliary transformer, and \textit{Paired} pretraining as used in \model setting.
\cx{fig TODO}.
}
	\label{fig:selflearn}
\end{figure}


==> Sections/8_notes.tex <==
\section{Notes}

Sec 1
seq-level corrective?
concise: abbreviation of i
abs: distracting? challenging?
compare with Electra's all mlm
name convention: base++ or more training data?

Sec 3
notation vector/scalar/matrix
X$_mlm$
Cor-LM? Mask-LM? Seq-CL? SCL?
Stop grad for all mlm copy

Sec 4 
model architecture shallow but same-width
equal training weight

\model{}

\cx{Motivation: We want go beyond token-level language model pretraining, why?
\begin{enumerate}
    \item No explicit guidance to learn sequence level representations, although many downstream tasks care more about representing the full sequence (sentence, passage, documents, etc.)
    \item A large amount Mask-LM or Auto-regresive LM is less informative: simple words, language synthetic, may limit the full potential of pretraining, as shown by the logarithmic scaling of model size versus effectiveness.
    \item Minnor: mismatch in pretraining input with [mask] and never full sentence, versus when applied.
\end{enumerate}
}


\cx{What we contribute in \model{}: Contrastive language REpresentation Pretraining by correcting text Sequences
\begin{enumerate}
    \item Built upon Electra's generator-style pretraining construction, leverage a PLM to provide corrupt sequences (PLM-Corruption) as pretraining data: thus elevate pretraining by focusing on PLMs' mistakes and also close the gap between pretraining input and application input.
    \item Bringing in the Contrastive Learning framework to enforce both sequence and token level denoising task: closely align the LM-corrupt sequence with transformed origin, while also efficient token level denoising pretraining task as replace token correction.
    \item Thorough study to show the effect of sequence level denoising and token level denoising. Sequence: uniformity in the representation space? Token: stronger training signal that guides transformers to learn more global/contextualized attention/representation?
\end{enumerate}
}


\cx{what experiments to show:
\begin{enumerate}
    \item Overall GLUE with Base and Base++, hopefully also GLUE Test
    \item Ablation study: Electra+rel-pos, shallow-gen-rel-pos, +Seq Contrast, +Token-Correction
    \item Influence of Token Level Denoising: different attention pattern? show learned replace token correction accuracy and replace acc?
    \item Influence of seq level denoising: the meaningfulness of [cls] with seq-contrast, the distribution/uniformity of learned [cls] in the representation space of pretraining data and on GLUE data? attention pattern to and from CLS?
\end{enumerate}}


\cx{What are the advantage of CREPES? What are the experiments to demonstrate its advantage?
\begin{enumerate}
    \item More Robust Pretraining: the contrast provides sequence level regularization that makes the pretraining more robust
    % \item Stronger pretraining signals: working on correcting LM's error boost the pretraining, stronger training signals in the end
    \item More global attention: push model leverage more contextual information. both correction tasks push the pretraining model learn more global information?
\end{enumerate}
How to demonstrate we have those advantages beyond overall effectiveness?
\begin{enumerate}
    \item {Robustness:} better few-shot performance on GLUE? better zero-shot performance in STS tasks? Show SVD/t-SNE of [CLS] on STS to show that the learned representation is more regularized?
    % \item {Stronger Pretraining:} ablation versus random corruption and fix generator.
    \item {More global attention:} visualize attention pattern? statistics of max attention path/how attention matrix scatters? Edge probing (maybe not)
\end{enumerate}
}

\cx{Experimental plan:
\begin{enumerate}
    \item Finish overall table (with base for now) (Chenyan), + SQuAd
    \item start ablation table and fill in (Yu design the table)
    \item (robustness) Few-shot glue (MNLI only?) (Yu code/script) (chenyan check preprocessing)
    \item (robustness) [CLS] space visualization (STS)
    \item (More contextualized) word's h self-similarity (pretrain data and downsteam, STS? MNLI?) (without stopword) https://arxiv.org/abs/1909.00512 self-sim, fig 2.
\end{enumerate}
}



\cx{Intro Outline, one bullet one paragraph:
\begin{enumerate}
    \item Language model is great and includes various different variations of token level LM pretraining tasks: MLM, Auto-regressive LM, the combination of the two, and other variations (rotation, permutation, etc.)
    \item Those tasks are great by not without limitations: 1) no explicit guidance of full sequence level---previous attempts often yield ambivalent empirical results in representation tasks. 2) Token level tasks are not all informative, while previous attempts to reweight/filter also show no general simple fix (salience span.. 3) mismatch between input seems in pretraining and those in applications. (Leave the more detailed discussion of previous attemtps in related work)
    \item This work presents our model. general idea, and describes each component
    \item more detail of our model
    \item experiments on GLUE, ablation study
    \item more insights on influences of seq level denoising and token level denoising
\end{enumerate}}

==> Sections/checklist.tex <==
% \newpage

\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We provide comprehensive evaluation results and comparison with prior work in Section~\ref{sec:eval} to validate the effectiveness of our proposed methods.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We provide discussions about the long training cycle and expensive costs of pretraining in Appendix~\ref{app:discussions}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendices~\ref{app:glue} and \ref{app:hyperstudy}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We report the median/average results of multiple random seeds, following previous studies. See Section~\ref{sec:setup}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Figure~\ref{fig:efficiency} and Appendix~\ref{app:hyper}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{sec:setup} and Appendix~\ref{app:glue}.}
  \item Did you mention the license of the assets?
    \answerNo{The license can be found in the original source of the assets.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> Tables/clm_ana.tex <==
\begin{wraptable}{r}{0.5\textwidth}
    \centering
    \vspace{-0.3cm}
%  \input{Tables/clm_sim_squad}
 \resizebox{\textwidth}{!}{
 \begin{tabular}{l|lll|ll}
\toprule 
% &\multicolumn{3}{c|}{\textbf{Analyses}} & \multicolumn{2}{c}{\textbf{SQuAD 2.0 DEV}} \\ \cline{2-6}
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Word Similarity}}  
& \multicolumn{2}{c}{\textbf{SQuAD 2.0 DEV}} 
\\ 
% \cline{2-6}
 & Self & Rand & Gap & EM & F1 \\
\midrule
% RoBERTa (Ours) & 0.781	&	0.603	&	0.178	& 77.71	& 80.51 & -- & -- \\ 
% ELECTRA (Ours) & 0.722	&	0.603	&	0.119 & -- & --	
%  \\ \hline
% RTD Only & 0.765 & 0.579 & 0.186 & 83.66 & 86.42 \\
\model  & 0.747 & 0.517 & \textbf{0.230}	& \textbf{83.96} & \textbf{86.79} \\
w.o. \clm & 0.832 & 0.724	& 0.108	& 83.63 & 86.48
 \\
\bottomrule
\end{tabular}
}
 
 \caption{The word similarity on MNLI corpus (pretrained, no fine-tuning) from \model (with and without CLM) and their SQuAD results. \textit{Self} is the average cosine similarity between the same word's $\bs{h}$ when appearing in different contexts~\cite{ethayarajh2019contextual}. \textit{Random} is that of two random words. Gap is their difference. 
 The analyses use the \textit{base++} setting for robust observations.
 } 
\label{tab:self_sim}
\end{wraptable}
   


==> Tables/clm_ana_back.tex <==

\begin{figure}\BottomFloatBoxes
   \begin{floatrow}
       \ttabbox{\resizebox{0.62\textwidth}{!}
         {\input{Tables/clm_sim_squad}}}
         {\caption{The word similarity test of different \model variations and their SQuAD results. The word similarity is the cosine similarity between representations of the same word in different contexts (Self), random word pairs (Random) and their Differences in MNLI corpus without fine-tuning.} 
\label{tab:self_sim}}
      \hspace{0.2cm} 
      \ffigbox[\FBwidth]{\raisebox{-1\height}
    {\caption{The entropy of attention weights across Transformer layers on MNLI without fine-tuning. The x-axis indexes the layer starting after embeddings.
    % (smaller means closer to input tokens). 
    % The entropy is averaged on all tokens in the MNLI corpus without fine-tuning.
    } 
    \label{fig:attn_study}
    }
    \includegraphics[width=0.3\textwidth]{Figures/attn_plot.pdf} \vspace{-0.3cm}
    }

\end{floatrow}
\end{figure}


==> Tables/self_sim.tex <==


\begingroup
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\small
\centering
\begin{tabular}{lccc|ccc}
\hline
& \multicolumn{3}{c|}{\textbf{All Words}} & \multicolumn{3}{c}{\textbf{Stop Words}}  \\ \hline
\textbf{Model} & Self & Rand. & Diff. & Self & Rand. & Diff. \\
\hline
RoBERTa & 0.781	&	0.603	&	0.178	&	0.812	&	0.664	&	0.148  \\ 
ELECTRA & 0.722	&	0.603	&	0.119	&	0.682	&	0.606	&	0.076
 \\ 
\hline
\model & 0.738	&	0.626	&	0.112	&	0.699	&	0.639	&	0.060
 \\
\quad CLM Only & 0.721	&	0.616	&	0.105	&	0.718	&	0.651	&	0.067
 \\
\quad SCL+RTD & 0.680	&	0.595	&	0.085	&	0.669	&	0.619	&	0.050
 \\
\hline
\end{tabular}
\caption{
Average cosine similarity between representations of the same word in different contexts (Self), random word pairs (Rand.) and their differences (Diff.) in MNLI corpus, without fine-tuning. 
\cx{We don't need the Stop Words columns. Replace them with SQuAD numbers. to show the correlation of token self sim with SQuAD performance.}
}
\label{tab:self_sim}
\end{table}

\setlength{\tabcolsep}{6pt}

